LoRA Soups: Merging LoRAs for Practical Skill Composition Tasks

Low-Rank Adaptation (LoRA) is a popular technique for parameter-efficient fine-tuning of Large Language Models (LLMs). We study how different LoRA modules can be merged to achieve skill composition -- testing the performance of the merged model on a target task that involves combining multiple skills, each skill coming from a single LoRA. This setup is favorable when it is difficult to obtain training data for the target task and when it can be decomposed into multiple skills. First, we identify practically occurring use-cases that can be studied under the realm of skill composition, e.g. solving hard math-word problems with code, creating a bot to answer questions on proprietary manuals or about domain-specialized corpora. Our main contribution is to show that concatenation of LoRAs (CAT), which optimally weights LoRAs that were individually trained on different skills, outperforms existing model- and data- merging techniques; for instance on math-word problems, CAT beats these methods by an average of 43% and 12% respectively. Thus, this paper advocates model merging as an efficient way to solve compositional tasks and underscores CAT as a simple, compute-friendly and effective procedure. To our knowledge, this is the first work demonstrating the superiority of model merging over data mixing for binary skill composition tasks. Code and data are available at https://github.com/aksh555/LoRA-Soups

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and precede the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Claims made in the abstract and introduction are based on the results we obtain and have been justified in \autoref{sec:experiments}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{sec:limitations}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not introduce theoretical proofs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{s:exp_details} and \autoref{appx:additional_exp_details} and provided supplementary zip file for code and data.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All code and data are provided in the supplementary zip file.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{s:exp_details} and \autoref{appx:additional_exp_details}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See \autoref{appx:math-word}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The compute used for our experiments and time consumed is provided in \autoref{appx:compute}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Anonymity preserved
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no societal impact of the work performed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: As such there are no risks as these are publicly available documents. We ensure their appropriateness and quality. See \autoref{appx:qa_data}
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All data sources, datasets, and models have been appropriately cited.
    \item[] Guidelines: 
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Documented in \autoref{appx:qa_data} and released (zip file attached).
    % \item[] Guidelines:
    % \begin{itemize}
    %     \item The answer NA means that the paper does not release new assets.
    %     \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
    %     \item The paper should discuss whether and how consent was obtained from people whose asset is used.
    %     \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    % \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> old_introduction.tex <==
\section{Introduction}
\label{sec:introduction}



Large Language Models (LLMs) have demonstrated impressive conversational skills and abilities at solving general-purpose tasks such as writing emails or answering commonsense questions. However, when used out-of-the-box, they struggle in scenarios requiring reasoning or specialized domain knowledge. One of the reasons for this failure is their lack of technical knowledge but above all, their limited ability to compose skills from multiple domains. This limits their practical application to fields like multi-hop reasoning \cite{yang2024large}, program synthesis \cite{austin2021program}, education \cite{chevalier2024language}, medicine \cite{wu2024pmc} or in-house chatbots. 



Recently, the most capable LLMs \cite{anthropicIntroducingNext,abdin2024phi,achiam2023gpt,llama3modelcard,jiang2023mistral,reid2024gemini} exhibit impressive results on these compositional tasks. One of the ingredients behind this success is the training over a mixture of a gigantic number of specialized datasets. This data mixture gathers internet data but also very expensive data acquisition where in-domain annotation is needed. Besides, even though training on such a mixture might bestow a large set of skills to the model, several works report that finetuning is still needed in practice to increase the model's performance on specialized tasks. And this need is independent of the scale. For instance, Code-Llama 70B \cite{roziere2023code} has been trained on additional 600B tokens compared to Llama2 70B \cite{touvron2023llama2} and improves the performance of this latter by 26.8\% on the Human-Eval dataset \cite{chen2021codex}. Therefore, even for large-scale models, finetuning on specialized datasets significantly improves the performance. However, such finetuning is very costly and entails task-annotation in that domain. Indeed, once the model is finetuned, it is specialized in a very specific skill(s). In order to adapt it to a new compositional task, one need to finetune the model again on a new set of specialized datasets. 

Recently, \emph{model merging} has appeared as a cheap alternative for solving compositional tasks. Given a set of models wherein each is specialized in a skill, we combine their weights to obtain a new model. This approach is cheap since in most cases it does not require any further training. Before being applied to compositionality, model merging was historically applied to improve the accuracy and robustness of computer vision models trained on a single task \cite{wortsman2022model}. Later on, several works \cite{ilharco2022editing,jin2022dataless,matena2022merging,yadav2023tiesmerging,yu2024language} used model merging to obtain decent out-of-domain generalization results. However, their merging techniques are heavy in that they need to combine \emph{all the parameters} and most of these works focus on problems with \emph{mild} distribution shift e.g.\ a set of models finetuned on QA datasets and test on a new QA dataset. 

More recently, a series of works \cite{gu2024mix,shah2023ziplora,yang2024lora} investigated the merging of LoRA modules (instead of full models) in computer vision. Their main application is image generation where they combine visual styles and concepts.  The use of LoRA in the context of model merging is appealing. Indeed, LoRA involves a much smaller set of parameters and requires updating only a few layers e.g.\ the query and value layers (instead of updating all the layers). 
The impressive image generation results are mainly due to the ease of identifying basic skills. Indeed, to generate an image, it is quite intuitive to define concepts that build the image e.g.\ cartoon line drawing, watercolor painting, etc. 

Similarly, sufficiently complex natural language tasks can also be viewed through a compositional lens, but the skills involved are much harder to identify, making the use of LoRA merging more challenging. Many papers \cite{buehler2024x,feng2024mixture,luo2024moelora,muqeeth2024learning,wu2023mole} have also considered this setting but with the objective of multitask learning, which aims to retain the knowledge of each submodel's skill. On the other hand, the skill composition paradigm -- which refers to the case where the models learn a few skills and then combine them at inference time to solve an out-of-distribution problem that requires these skills-- is understudied. Huang et al.\ \cite{huang2023lorahub} show that by combining models finetuned on FLAN \cite{longpre2023flan}, they achieve high performance on Big-Bench Hard (BBH) \cite{suzgun2022challenging}. However, their distribution shift is mild in that the tasks in FLAN and BBH are very similar and the tasks are not necessarily compositional, i.e. the base model with few-shot prompting itself performs equivalently to their composing strategy. Akiba et al.\ \cite{akiba2024evolutionary} propose an evolutionary algorithm for merging LoRAs specialized in Japanese and in math \cite{cobbe2021training} to solve word-math problems in Japanese \cite{shi2022language}. However, their study is limited to this sole skill composition task.

In this paper, we investigate the use of LoRA merging for solving skill composition tasks when the number of skills is 2. Compared to prior work, we study a wider range of skill composition tasks with larger distribution shifts e.g.\ solving math problems with code and answering questions about narrow domains, these are harder tasks where few-shot prompting performs poorly. We introduce Learnable Concatenation (\textbf{CAT}), a simple merging scheme that consists of a weighted average of the LoRA updates. Though we learn these weights in CAT for knowledge retention on the individual skills themselves, we observe the emergence of the ability to solve such compositional problems. It not only beats many existing merging algorithms but also outperforms a model that has been finetuned on the mixture of datasets (we refer to this model as \textbf{DATA-MIX}). DATA-MIX is also not straightforward when the data styles are different making training hard and also the output does not necessarily conform to the desired format. To our knowledge, our work is the first to show that model merging outperforms data merging. 

Another highlight of our results is that \textbf{CAT} achieves a super-linear improvement when solving word-math problems with code i.e.\ the set of problems solved by \textbf{CAT} is strictly larger than the set of problems solved by the math model or by the code model.



Our key contributions are summarized as follows:
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt]
    \item[--] We define the skill composition problem and show some practical applications in domains spanning code, science, robustness, and in-house use cases in \autoref{sec:setting}. 
    \item[--] We introduce Learnable Concatenation (\textbf{CAT}), a LoRA merging technique that involves a simple weighted average of the encompassed skill LoRAs. While LoRA concatenation as a technique already exists, our contribution lies in learning the weights assigned to each skill and applying it to compositional natural language tasks.
    \item[--] We perform a comprehensive evaluation of several baselines in \autoref{sec:experiments} and demonstrate that \textbf{CAT} achieves better skill composition than not only existing merging methods but also beats the most expensive method \textbf{DATA-MIX}, which finetunes a model on a mixture of skill-specific datasets. Finally in \autoref{sec:limitations}, we discuss some limitations of our approach.
\end{itemize}

































\newpage




Don't forget to talk about the advantage of LoRA based merging + that LoRA based merging is different from computer vision


there are models that are towards AGI like GPT-4. On the other hand, finetuning models get you very narrow but very good. Suppose we finetune those models on narrow doamins can we combine the small models to get the best all of worlds? Doing a mix of datasets this is a naive approach. Other methods and enssemble . Historically, mix datasets is best method. But our contribution we show that we are doing by combining models. 

We found out clever mix generalize to other ssskill mix where mixing data is very hard (like the chatbot or reading comprehension). 




\vspace{2cm}

\begin{itemize}
  \item[--] we want skill composition. justify why skill composition is interesting to achieve.
  \item[--] the way of OpenAi is getting: train on all possible data. union of all skills. generate all the data that has all skills.
  \item[--] it is ok if you are openai. there are a lot of cases when FT is helpful for specialized skills even for very large models, FT gets you strong performance. For instance, code llama, llema. Finetuning on specific data helps you achieve stronger skills. Even for these models and big models trained on whole internet, FT helps. 
  \item[--] FT on large models make you strong. The problem is that you get agent that is very strong in very specific task. Models become specialized. But the problem is that for skill composition it is very expensive, we would have to retrain the model. Now i want to solve a problem that combines skills. I finetune on dataset . Every skill compoition I want to come up with, I need to retrain a model. 
  \item[--] Another solution is to get models that are specialized and combien them. It is of course more efficient and we show we get better results.
\end{itemize}

==> old_setting.tex <==
\section{Setting}
\label{sec:setting}


In this section, we present the skill composition problem and some instances where it appears. Then, we discuss various methods to learn skill composition. Finally, we introduce some skill composition problems that are of scientific and practical interests.


\subsection{Skill composition}

Natural language tasks may always be decomposed into a set of basic skills. In this paper, we refer to a skill as a subtask that is necessary to complete a global task. The definition and number of these skills control the complexity of the task. Easier problems often require mastering a fewer and simpler skills,  and may require less compute to find the answer. By contrast, complex problems require to master a large number of skills and entail more compute to solve. While the precise definition of skills is not always guaranteed in a given task, we focus on natural language tasks where composition can be ensured and isolated (see \autoref{sec:problems} for examples).

\todo{EM: I think the following paragraph is mixing between the problem, which is learning to compose skills that appear in separate datasets, and the solution - model merging. You can actually introduce the skill composition problem without discussing model merging, right?}
The skill composition problem consists of a global task that may be clearly decomposed in two (or more) distinct subtasks. We train one submodel per subtask and at test time \todo{EM: is this really at test time?}, we merge them and evaluate the resulting model on the global task. A description of the most used \todo{most commonly used? or just, previous} merging strategies is provided in \autoref{sec:merging}. A merged model is successful if it is able to perform better than each individual model\todo{EM: why is beating the individual models the right baseline?} and should be able to use each skill at the right time when completing the global task. For instance, when solving a math-word problem, the model should first write the reasoning and then write some code to perform the calculations.

Skill composition is challenging since it is not clear that the merged model understands which skill to use at test time. It is possible that the new skills confuse it\todo{use a better term} and this results in worse performance compared to the initial model. In this paper, we show that by using simple merging schemes, we can achieve high performance on compositional tasks and observe that the merged model uses each skill at the right place\todo{sounds a bit weird, maybe uses each skill correctly?}.




\subsection{Merging methods}\label{sec:merging}


The ability of models to compose skills is primarily attributed to the merging method. Given a set of models such that each one is trained on a skill, a merging method is a recipe to combine these weights \cite{wortsman2022model}. In this section, we review the different merging schemes and report their skill composition performance in the next sections. 

\todo{The "common ground" paragraph is confusing, maybe make clear that you are introducing LoRA here and not a LoRA merging method. Maybe put in a separate paragraph without bold font, start with "Before we describe LoRA merging methods, ..."}
\paragraph{Common ground.} All the methods are based on the LoRA  technique \cite{hu2021lora} that is defined as follows. During finetuning, the update of the weights are constrained to be a low-rank decomposition i.e.\  the update is $W_0+\Delta W$, where $\Delta W= BA^{\top}$, for $B\in\mathbb{R}^{d\times r},$ $A\in\mathbb{R}^{d\times r}$, and $r\ll d.$ During training, $W_0$ is frozen and $A$ and $B$ are trainable. Therefore, for a task that requires $k$ skills, we train LoRA parameters for each skill, resulting in $k$ pairs of LoRA parameters $(A_1,B_1),\dots,(A_k,B_k).$ For the sake of simplicity, we consider $k=2$ in our explanations. We next detail how to combine these LoRA parameters to obtain skill composition.


%https://huggingface.co/blog/peft_merging#concatenation-cat


\paragraph{Concatenation of LoRAs (CAT).} This method consists in a weighted concatenation of the LoRA modules i.e. $\Delta W = B_{cat} A_{cat}^{\top}$, where $B_{cat}=[\alpha_1B_1,\alpha_2B_2]\in\mathbb{R}^{d\times 2r}$ and $A_{cat}=[A_1,A_2]\in\mathbb{R}^{d\times 2r}.$ \todo{isn't it simpler to write is as $\Delta W_{\mathrm{cat}} = \alpha_1 \Delta W_1 + \alpha_2 \Delta W_2$?}The merging coefficients $\alpha_1,\alpha_2 >0$\todo{probably minor, but are you enforcing this in the optimization?}  control the contribution of each LoRA module and set them to trainable parameters. In summary, the training procedure is as follows: 1) we train each of the LoRA modules separately on each skill 2) We freeze the previously trained LoRA modules and train the merging coefficients on a dataset that mixes the skills.\todo{this pipeline sort-of applies to all LORA merging methods, no?} While the concatenation of LoRAs has been used in the literature \cite{peft}, one of our contributions is to finetune the merging coefficients. \todo{EM: I thought some of the experiments suggested that this is not always helpful...}

\paragraph{MoE of LoRAs (MoE).} 

\paragraph{TIES.} TrIm, Elect Sign, and Merge (TIES\todo{TIES-MERGE?}) \cite{yadav2024ties} is a three-step method for merging models. First, we ``trim'' the LoRA parameters, i.e.\ we prune the smallest values of $(A_k,B_k)$ for $k\in\{1,2\}$ and retain the top values based on the specified density fraction $\lambda\in[0,1].$ Then, we ``elect'', i.e.\ we calculate the majority sign mask from the pruned LoRA weights by summing all their parameter values and storing the sign of this sum. Lastly, the LoRA weights are multiplied by weights $(\alpha_1,\alpha_2)$, followed by a disjoint merging based on the majority sign mask. \todo{it's not very clear to me, does the rank increase here?} In this process, $(\lambda,\alpha_1,\alpha_2)$ are hyperparameters to be tuned.



\paragraph{DARE.} Drop And REscale (DARE) \cite{yu2023language} consists in two steps. Similarly to TIES, we first randomly prune the values of the LoRA parameters $(A_k,B_k)$ for $k\in\{1,2\}$ based on a density $\lambda\in[0,1]$. Then, we rescale the pruned LoRA weights by $1/\lambda$ which yields  $(A_k^{(DARE)},B_k^{(DARE)})$. Lastly, we apply a linear merging i.e.\ $\Delta W = (\alpha_1B_1^{(DARE)}+\alpha_2B_2^{(DARE)})(A_1^{(DARE)}+A_2^{(DARE)})^{\top}$.\todo{do they add the cross-products here?} Similarly to TIES,  $(\lambda,\alpha_1,\alpha_2)$ are  also hyperparameters to be tuned.


%https://matilabs.ai/2024/03/05/slerp-model-merging-primer/#slerp

\paragraph{SLERP.} Spherical LinEar inteRPolation (SLERP) \cite{Digitous2023Digitous,shoemake1985animating} is an interpolation technique that merges two models on the spherical plane. To create the merging coefficients $\alpha_1$ and $\alpha_2$, we first normalize the $A_k$'s i.e.\ $\overline{B_kA_k} = B_k{A}_k/\|B_kA_k\|_2$ for $k\in \{1,2\}.$ Then, we compute $\theta_{BA} = \mathrm{arccos}\left(\mathrm{sum}((\overline{B_1A_1})\odot (\overline{B_2A_2})\right)$ and defined the merging coefficients as:
\begin{align}
   \alpha_1^{(SLERP)} = \frac{\sin\left((1-t)\theta_{BA}\right)}{\sin(\theta_{BA})}, \qquad \alpha_2^{(SLERP)} = \frac{\sin\left(t\cdot\theta_{BA}\right)}{\sin(\theta_{BA})},
\end{align}
\mbox{for $t\in[0,1]$ hyperparameter to be tuned. The update is $\Delta W = \alpha_1^{(SLERP)} B_1A_1 + \alpha_2^{(SLERP)} B_2A_2$.} We remark that SLERP is similar to CAT but differ by the parametrization of the merging coefficients.


\todo{I wonder if there's a general way to capture all these methods, like they all do some operation on the individual LoRAs, compute the coefficients, and then average the LoRAs?}

\paragraph{Data mixing (DATA-MIX).} This method does not merge models but merges datasets. We fine-tune a \emph{single} model with LoRA weights $(A,B)$ where $A,B\in\mathbb{R}^{d\times kr}$ on the concatenation of datasets and thus simultaneously teach the $k$ skills to the model. We set the rank to $kr$ (and not $r$) in order to ensure a fair comparison with the other merging methods. DATA-MIX is an important baseline since it has outperformed merging methods such as TIES or DARE in the multi-task case. Besides, one of the contributions of this paper is to understand when model merging beats data mixing. \todo{it is weird that this appears in the LoRA merging section}

%a remark on previous merging papers are on 


\subsection{Skill composition problems}\label{sec:problems}


Most of prior work on model merging has focused on knowledge retention. This latter assumes that we have one model per skill. We then merge these models and hope that the resulting model does not forget its knowledge and still does well on each of the skills. In this work, we mainly focus on \emph{skill composition}. This problem has not been explored in the context of model merging and is more challenging than knowledge retention since it is an out-of-distribution setting. In this section, we propose novel skill composition problems where we evaluate our model and data merging methods

\paragraph{Hard math-word problems.} Prior works noticed that when fine-tuning a large language model on GSM-8k \cite{cobbe2021training}, the resulting model performs poorly on GSM-Hard \cite{gao2023pal}, a dataset that gathers similar problems but with more complex arithmetic operations. The program-aided approach by Gao et al.\  \cite{gao2023pal} is one solution to address this issue: the LLM reads the GSM problem and generates programs as the intermediate
reasoning steps, but offloads the solution step to a Python interpreter. Therefore, in order to improve the accuracy on GSM-hard, we set the first skill to be MetaMathQA \cite{yu2023metamath} --an augmented version of the GSM-8k dataset-- and the second skill to be Code-Alpaca \cite{codealpaca}. In \autoref{sec:math_code}, we show that both data and model merging create models that master math and code and that are able to use each skill at the right place.

\paragraph{Prompt robustness.}  Recently, a few works \cite{mizrahi2024state,sclar2024quantifying} report the sensitivity of language models to prompt formatting. These works report performance differences of up
to 76 accuracy points due to subtle changes
in prompt formatting when using LLaMA-2-13B \cite{touvron2023llama}. This sensitivity remains when increasing model size, the number of few-shot examples, or performing instruction tuning. We investigate whether model or data mixing is a solution to this problem. We consider a task where the input is a sentence and the model is asked the following question "How many words contain the letter 'o' in the sentence?". For this task, Sclar et al.\ \cite{sclar2024quantifying} provide 10 datasets of 6000 examples containing the same sentences but differ by their format. Examples of formats are the upper case format i.e.\ "SENTENCE", "ANSWER" or the $\texttt{\textbackslash n}$ format i.e.\ "Sentence$\texttt{\textbackslash n}$", "Answer$\texttt{\textbackslash n}$". Therefore, we set the first skill to be the dataset with format $i$ and the second skill to be the dataset with format $j$ and evaluate the merging methods on a dataset with format $k$, where $i,j,k\in\{1,\dots,10\}$ and $i\neq j\neq k.$ In \autoref{sec:prompt_robustness}, we show that merging models improves the robustness to prompt formatting changes.

\paragraph{Chatbot on proprietary manuals.}  Chat models are language models that aim to facilitate conversational interactions. Similarly to LLMs, they are first pre-trained on large language datasets. Then, they are finetuned on instruction-tuning datasets  \cite{vicuna2023,conover2023free,kopf2024openassistant,alpaca,xu2023baize,xu2023wizardlm,zhou2024lima}. While general-purpose chatbots are useful, an institution or corporation may desire to have a \emph{specialized} chatbot that addresses domain-specific questions. Examples of this case may be a university that wants a chatbot that answers questions about quantum physics or a refrigerator retailer that wants a chatbot to answer questions about their last device. The aforementioned approach may fall short since when fine-tuning a chat model on a specialized document, it may lose its conversational abilities. Another solution would be to obtain an instruction-tuning dataset that covers the specialized material but this may too costly. On the other hand, model merging seems to be convenient solution to address this problem: we train one LoRA model on a general instruction-tuning dataset and another one on the specialized document. Therefore, we set the first skill to be the Alpaca dataset \cite{alpaca} and study two cases: when the second skill is a molecular biology textbook \cite{bergtrom2022basic} and when it is a manual of the "Dungeons and Dragons" game \cite{gygax1974dungeons}. \textcolor{orange}{In \autoref{sec:chatbot}, we show that LoRA merging  yields specialized chatbots that beat several reasonable baselines.} 

%One may want to use language model to answer questions about text corpus in a specific domain such as in medicine or in law.

\paragraph{Reading comprehension on technical documents.} Medical reports and law contracts are very challenging to read for non-specialist users: they are usually very long and  involve a myriad of technical words. Having a language model that can read these documents and answer questions may give may be very useful. For this reason, we train one LoRA model on SQuAD \cite{rajpurkar2018know} to acquire the reading comprehension skill and another LoRA on biology textbooks \cite{grewal2023human,klymkowskybiofundamentals,nelson2021medical,singh2014genetics}. We test our models on the BioASQ-QA dataset \cite{krithara2023bioasq}, a reading comprehension dataset on biomedical engineering. In \autoref{sec:reading_comprehension}, we show that thanks to LoRA merging, the model is able to much better understand the technical words and thus make adequate answers. 




\subsection{Experimental setup}

In this section, we present our setup for the experiments in Sections \ref{sec:math_code}, \ref{sec:prompt_robustness}, \ref{sec:chatbot}, \ref{sec:reading_comprehension}.

\paragraph{Datasets.} We divide our training datasets into two categories: the instruction datasets, that have an instruction and an answer. This covers in our case, MetaMathQA, the datasets with different prompt formats from Sclar et al.\ \cite{sclar2024quantifying}, Alpaca and SQuAD; and the standard datasets, which contain just plain text like the biology textbooks in our case.



\paragraph{LoRA configuration.} Our base model is a Llama-7b \cite{touvron2023llama} and set the LoRA rank $r=32$, LoRA alpha $ = 64$, LoRA dropout $ = 0.05$ and the target modules to be $\texttt{\{"q\_proj", "v\_proj", "k\_proj", "up\_proj","down\_proj"\}}$. In the specific case of DATA-MIX, we train LoRA modules with a rank $2r=64$, to ensure an equal number of trainable parameters with the model merging methods.

\paragraph{Finetuning.} We finetune the individual LoRAs using AdamW \cite{loshchilov2017decoupled} for $3$ epochs, with a learning rate $3\mathrm{e}{-4}$, $100$ warmup steps, a linear decaying schedule, batch size in $\{4,8\}$ and gradient accumulation $4$. We set the precision to $\texttt{float16}$. Our loss is the standard next-token prediction loss. When finetuning on the instruction datasets, we mask the instruction so that we only penalize wrong token predictions at the level of answers. When finetuning on textbooks, we do not apply any masking.
\todo{MoE - We followed the implementation of \textit{mergoo} \cite{}.} 

\paragraph{CAT finetuning.} We add a finetuning step to learn the merging coefficients $\alpha_1,\alpha_2$. We freeze the trained LoRA modules and train $\alpha_1,\alpha_2$ on a dataset made by selecting the minimum of $5\%$ of the data points from both skill 1 and skill 2. This additional step only runs for $1$ epoch with a learning rate of $1\mathrm{e}{-4}$.
\todo{Best models in fine-tuning chosen by taking the best model on the validation set.}

\paragraph{Hyperparameters.} \todo{TIES, DARE: implemented using PEFT \cite{} and choosing values by doing sweep over $\lambda \in [0,1], \alpha_1 \in [1,2], \alpha_2 \in [1,2]$.}

\paragraph{Evaluation.} At inference time, we generate answers in an autoregressive fashion with \texttt{temperature} $0$, \texttt{max\_new\_tokens} $200$, with nucleus sampling probability \texttt{top\_p} as $0.95$. In \autoref{sec:math_code}, we consider a text-only generation as correct if the final result matches with ground truth. Alternately, a code-generation is correct if a Python interpreter can execute it. In Sections \ref{sec:prompt_robustness} and \ref{sec:chatbot}, a generation is correct if it matches with ground truth. In \autoref{sec:reading_comprehension}, because the exact matching and F1 scores do not capture the difference between models, we use GPT-4 as a judge \cite{zheng2024judging}. We ask it to compare all the pairs of answers with each other. The best model is the one achieving the highest ELO rating \cite{elo1978rating}.



\paragraph{Evaluation datasets.} We now detail our evaluation datasets in Sections \ref{sec:chatbot} and \ref{sec:reading_comprehension}.
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt]
    \item[--] For evaluating prompt format robustness in \autoref{sec:prompt_robustness}, we choose \texttt{task\_131} of counting the number of words having a particular letter in the given sentence from Super-NaturalInstructions \cite{supernaturalinstructions}. Following the grammar over \textit{descriptors}, \textit{separators}, and \textit{spaces} defined in \cite{sclar2024quantifying}, we sample 7 prompt formats. \todo{show the formats in a small table}
    \item[--] In \autoref{sec:chatbot}, we create question-answer datasets to evaluate our chatbots. We give random text excerpts from the textbooks/manuals and asking GPT-4  \cite{achiam2023gpt} to generate a question and answer pair. Each of these evaluation methods contains 50 questions.
    \item[--] In \autoref{sec:reading_comprehension}, we restrict the BioASQ dataset to questions with a context length smaller than 500 tokens. Indeed, we observed that the model suffers from length generalization: when the context length much larger than the one seen during training, the model does not output any answer. Lastly, we restrict the type of questions to "factoids", in order to align with the type of questions in SQuAD. This data processing results in 200 questions.

\end{itemize}


{
\color{red}
Missing things: evaluation with 8-shot PAL for section 3


}

==> plan.tex <==
% \section{Skill composition with LoRA merging}

There are all these LoRA merging models they show that they can retain knowledge but in practice what you care about is actually mixing skills to solve new tasks. And so the question we address in this paper is: can these lora merging solve tasks that require 2 skills? (some people did it before but it's not their main focus)


\begin{itemize}
 \item[--] 1) Setting
 \begin{itemize}
    \item[$\ast$] Describe problem formulation
    \item[$\ast$] Describe all the merging methods (like we did for the posistional encodings in the Length generalization paper)
    \begin{itemize}
       \item[$\bullet$] Learned CAT
       \item[$\bullet$] TIES
       \item[$\bullet$] DARE
       \item[$\bullet$] SLERP
       \item[$\bullet$] MoE of LoRAs
    \end{itemize}
    \end{itemize}
\item[--] 2) Prompt formats
    
\item[--] 3) Math + code
\item[--] 4) Question answering (chatbot): molecular biology + boardgame
\item[--] 5) Reading comprehension (biology)
\item[--]
\end{itemize}

First thing to say: Learned CAT beating the data mixture 

With data has very different distributions tails, LoRa merging is the best thing to do

Experiment: Dataset with different categories/labels and train MoE with different system prompt

Explain why F1 score is bad
